Manipulating UAV Imagery for Satellite Model Training, Calibration and Testing

Modern livestock farming is increasingly data driven and frequently relies on efficient remote sensing to gather data over wide areas. High resolution satellite imagery is one such data source, which is becoming more accessible for farmers as coverage increases and cost falls. Such images can be used to detect and track animals, monitor pasture changes, and understand land use. Many of the data driven models being applied to these tasks require ground truthing at resolutions higher than satellites can provide. Simultaneously, there is a lack of available aerial imagery focused on farmland changes that occur over days or weeks, such as herd movement. With this goal in mind, we present a new multi-temporal dataset of high resolution UAV imagery which is artificially degraded to match satellite data quality. An empirical blurring metric is used to calibrate the degradation process against actual satellite imagery of the area. UAV surveys were flown repeatedly over several weeks, for specific farm locations. This 5cm/pixel data is sufficiently high resolution to accurately ground truth cattle locations, and other factors such as grass cover. From 33 wide area UAV surveys, 1869 patches were extracted and artificially degraded using an accurate satellite optical model to simulate satellite data. Geographic patches from multiple time periods are aligned and presented as sets, providing a multi-temporal dataset that can be used for detecting changes on farms. The geo-referenced images and 27,853 manually annotated cattle labels are made publicly available.

==> ManipulatingDroneImagery (2)/table_Flights.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Designation} & \textbf{Location} & \textbf{Date Range} & \textbf{\begin{tabular}[c]{@{}c@{}}Number \\ of \\ Flights\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number \\ of \\ Images\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number \\ of Patch \\ Pairs\end{tabular}} \\ \hline
A1-A15 & Highlands A & 15/7/2021-17/9/2021 & 15 & 5166 & 2726 \\ \hline
B1-B4 & Highlands B & 20/8/2021-31/8/2021 & 4 & 529 & 52 \\ \hline
C1-C5 & Highlands C & 10/9/2021-17/9/2021 & 5 & 1050 & 162 \\ \hline
PA1-PA3 & Sydney A & 15/7/2021-15/7/2021 & 3 & 384 & 76 \\ \hline
PB1-PB3 & Sydney B & 17/8/2021-19/8/2021 & 3 & 505 & 60 \\ \hline
PC1-PC3 & Sydney C & 7/9/2021-9/9/2021 & 3 & 142 & 12 \\ \hline
\textbf{Total} &  & 15/7/2021-17/9/2021 & 33 & 7776 & 3088 \\ \hline
\end{tabular}%
}
\caption{Details of all UAV flights.} 
\label{tab:flights}
\end{table}

==> ManipulatingDroneImagery (2)/table_augmentations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Function} & \textbf{Description} & \textbf{Parameters} \\ \hline
Rotate & \begin{tabular}[c]{@{}c@{}}Rotate pair by amount sampled \\ uniformly from {[}min,max{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}min, most negative \\ rotation amount\\ max, most positive \\ rotation amount\end{tabular} \\ \hline
Alignment & \begin{tabular}[c]{@{}c@{}}Shift only one of the image \\ pair slightly to create misalignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}shift standard deviation, \\ where shift is pixel amount \\ sampled from a zero mean Gaussian\end{tabular} \\ \hline
Shift & Shift pair of images together & \begin{tabular}[c]{@{}c@{}}shift standard deviation, \\ where shift is pixel amount \\ sampled from a zero mean Gaussian\end{tabular} \\ \hline
Colour & \begin{tabular}[c]{@{}c@{}}Shift each channel in RGB \\ colour space to recolour image\end{tabular} & \begin{tabular}[c]{@{}c@{}}shift standard deviation, \\ shift is {[}-255,255{]} and sampled \\ from a zero mean Gaussian\end{tabular} \\ \hline
Hue & \begin{tabular}[c]{@{}c@{}}Shift the image hue in HSV \\ colour space to recolour the image\end{tabular} & \begin{tabular}[c]{@{}c@{}}shift standard deviation, \\ shift is {[}-255,255{]} and sampled \\ from a zero mean Gaussian\end{tabular} \\ \hline
Saturation & \begin{tabular}[c]{@{}c@{}}Shift the image saturation \\ in HSV colour space\end{tabular} & \begin{tabular}[c]{@{}c@{}}shift standard deviation, \\ shift is {[}-255,255{]} and sampled \\ from a zero mean Gaussian\end{tabular} \\ \hline
Value & \begin{tabular}[c]{@{}c@{}}Shift the image value in \\ HSV colour space\end{tabular} & \begin{tabular}[c]{@{}c@{}}shift standard deviation, \\ shift is {[}-255,255{]} and sampled \\ from a zero mean Gaussian\end{tabular} \\ \hline
Mirror & \begin{tabular}[c]{@{}c@{}}Flip pair up/down and left/right. \\ Chance of each flip type is \\ sampled independently.\end{tabular} & \begin{tabular}[c]{@{}c@{}}probability, modeled as one Bernoulli \\ distribution for up/down and \\ another for left/right\end{tabular} \\ \hline
Scale & Scale pair by a random amount. & \begin{tabular}[c]{@{}c@{}}scale ratio standard deviation, \\ sampled from a zero mean Gaussian\end{tabular} \\ \hline
Noise & \begin{tabular}[c]{@{}c@{}}Add independent random noise \\ to each image pixel\end{tabular} & \begin{tabular}[c]{@{}c@{}}noise standard deviation, \\ noise is {[}-255,255{]}x3 and \\ sampled from a zero mean Gaussian\end{tabular} \\ \hline
Shear & \begin{tabular}[c]{@{}c@{}}Apply a shear geometric \\ operation to pair\end{tabular} & \begin{tabular}[c]{@{}c@{}}shear standard deviation, \\ shear is a ratio sampled \\ from a zero mean Gaussian\end{tabular} \\ \hline
Local Warp & See Above & \begin{tabular}[c]{@{}c@{}}max surface height and \\ warp together or independently\end{tabular} \\ \hline
\end{tabular}%
}
\caption{The augmentation functions provided, their effect on the image patch pair and the tuning parameters for each.}
\label{tab:augmentation}
\end{table}
